Testing DNN Image Classifiers for Confusion & Bias Errors

Image classifiers are an important component of today's software, from consumer and business applications to safety-critical domains. The advent of Deep Neural Networks (DNNs) is the key catalyst behind such wide-spread success. However, wide adoption comes with serious concerns about the robustness of software systems dependent on DNNs for image classification, as several severe erroneous behaviors have been reported under sensitive and critical circumstances. We argue that developers need to rigorously test their software's image classifiers and delay deployment until acceptable. We present an approach to testing image classifier robustness based on class property violations. We found that many of the reported erroneous cases in popular DNN image classifiers occur because the trained models confuse one class with another or show biases towards some classes over others. These bugs usually violate some class properties of one or more of those classes. Most DNN testing techniques focus on per-image violations, so fail to detect class-level confusions or biases. We developed a testing technique to automatically detect class-based confusion and bias errors in DNN-driven image classification software. We evaluated our implementation, DeepInspect, on several popular image classifiers with precision up to 100% (avg.~72.6%) for confusion errors, and up to 84.3% (avg.~66.8%) for bias errors. DeepInspect found hundreds of classification mistakes in widely-used models, many exposing errors indicating confusion or bias.

==> Makefile <==
# $Id: Makefile 1833 2006-06-19 21:51:36Z witchel $

.SUFFIXES: .fig .dvi .ps .pdf

VERSION = 0.0

#----------------------------------------------------------------------
# Source files.  Edit these variables for each new paper.
#----------------------------------------------------------------------

name = main

all: pdf bib

#----------------------------------------------------------------------
# LaTeX commands.
#----------------------------------------------------------------------

%.dvi:%.tex
	pdflatex $<

dvi: $(name).tex *.tex
	pdflatex $<

rub: $(name).tex 
	rubber -Wrefs -Wmisc $(name)

twice:
	pdflatex $(name)
	pdflatex $(name)

bib:
	bibtex $(name)
	pdflatex $(name)
	pdflatex $(name)


latex_junk = 	$(name).dvi \
		*.aux \
		*.log \
		$(name).blg \
		$(name).toc \
		$(name).out \
		psfig.aux \
		*.bbl \
		*.pdfsync \
		*.fdb_latexmk \
		*.fls \
		*.synctex.gz


#----------------------------------------------------------------------
# Postscript/PDF generation.
#----------------------------------------------------------------------

$(name).ps:
ps: $(name).dvi *.tex
	latex $(name).tex && latex $(name).tex
	$(DVIPS) -P pdf -t letter -o $(name).ps $(name).dvi

summary: summary.dvi

#DVIPS = dvips
DVIPS = dvips

%.ps:%.dvi
	$(DVIPS) -P pdf -t letter -o $@ $<

%.ps2:%.dvi
	$(DVIPS) -t letter -o ps2.tmp -p 2 $<
	mpage -2 -P ps2.tmp > $@
	rm ps2.tmp

pdf: 
	pdflatex $(name).tex

# DISTILL = distill
DISTILL_FLAGS = -embedallfonts on -maxsubsetpct 100

DISTILL = ps2pdf
#DISTILL_FLAGS =

%.pdf:%.ps
	$(DISTILL) $(DISTILL_FLAGS) $<

#----------------------------------------------------------------------
# Document previewers.
#----------------------------------------------------------------------

x:
	xdvi -s 5 $(name) &

gv: $(name).ps
	ghostview $(name).ps &


# Garbage files.
junk = $(latex_junk) *.ps *.pdf *.out


#----------------------------------------------------------------------
# Miscellaneous.
#----------------------------------------------------------------------

tags:
	etags $(latex_files)

clean:
	rm -f $(junk)

count:
	wc $(latex_files)


==> tables/bias-precision-recall.tex <==
% \begin{table}[!phtb]
% \centering
% \scriptsize
% %\caption{\textbf{\small Accuracy in bias bug detection for different models and datasets}}
% \caption{\textbf{\small Accuracy in confusion bias bug detection for different models and datasets}}
% \label{tab:bias_confusion_accuracy}
% %\begin{tabular}{l|l|cccccc}
% \begin{tabular}{l|l|rrrrrr}
% \toprule
% \multirow{4}{*}{\coco}  & threshold & 0.005 & 0.01 & \textcolor{red}{\underline{0.015}} & 0.02 & 0.025 & 0.03 \\
%  & precision & 0.63 & 0.73 & \textcolor{red}{\underline{0.84}} & 0.91 & 0.96 & 0.97 \\
%  & recall & 1.00 & 0.99 & \textcolor{red}{\underline{0.92}} & 0.79 & 0.62 & 0.48 \\
%  & \#TP & 1874 & 1852 & \textcolor{red}{\underline{1732}} & 1482 & 1162 & 897 \\

% \midrule
% \coco  & threshold & 0.005 & 0.01 & \textcolor{red}{\underline{0.015}} & 0.02 & 0.025 & 0.03 \\
% with & precision & 0.59 & 0.68 & \textcolor{red}{\underline{0.79}} & 0.87 & 0.94 & 0.98 \\
% gender & recall & 1.00 & 0.98 & \textcolor{red}{\underline{0.91}} & 0.78 & 0.62 & 0.46 \\
%  & \#TP & 1813 & 1769 & \textcolor{red}{\underline{1645}} & 1406 & 1123 & 831 \\

% \midrule
% imSitu  & threshold & 0.005 & 0.01 & 0.015 & 0.02 & \textcolor{red}{\underline{0.025}} & 0.03 \\
%  & precision & 0.18 & 0.30 & 0.50 & 0.71 & \textcolor{red}{\underline{0.88}} & 0.96 \\
%  & recall & 1.00 & 0.99 & 0.92 & 0.82 & \textcolor{red}{\underline{0.72}} & 0.61 \\
%  & \#TP & 739 & 730 & 679 & 611 & \textcolor{red}{\underline{535}} & 454 \\

% \midrule                
% \multirow{3}{*}{NUS}  & threshold & 0.001 & \textcolor{red}{\underline{0.002}} & 0.003 & 0.004 & 0.005 & 0.006 \\
%  & precision & 0.13 & \textcolor{red}{\underline{0.30}} & 0.51 & 0.65 & 0.73 & 0.87 \\
%  & recall & 1.00 & \textcolor{red}{\underline{0.91}} & 0.66 & 0.39 & 0.20 & 0.09 \\
%  & \#TP & 18765 & \textcolor{red}{\underline{17133}} & 12318 & 7301 & 3697 & 1610 \\

% \midrule
% \multirow{3}{*}{ImageNet} & threshold & \textcolor{red}{\underline{0.001}} & 0.002 & 0.003 & 0.004 & 0.005 & 0.006 \\
%  & precision & \textcolor{red}{\underline{0.02}} & 0.03 & 0.05 & 0.07 & 0.11 & 0.17 \\
%  & recall & \textcolor{red}{\underline{1.00}} & 0.93 & 0.69 & 0.38 & 0.18 & 0.07 \\
%  & \#TP & \textcolor{red}{\underline{9243}} & 8645 & 6358 & 3542 & 1627 & 647 \\

% \midrule
% \multirow{3}{*}{\cifar}  & threshold & 0.005 & 0.01 & 0.015 & \textcolor{red}{\underline{0.02}} & 0.025 & 0.03 \\
%  & precision & 0.10 & 0.12 & 0.17 & \textcolor{red}{\underline{0.27}} & 0.43 & 0.65 \\
%  & recall & 1.00 & 0.99 & 0.97 & \textcolor{red}{\underline{0.89}} & 0.56 & 0.20 \\
%  & \#TP & 474 & 471 & 458 & \textcolor{red}{\underline{421}} & 266 & 95 \\



% \midrule
% Robust& threshold & 0.02 & \textcolor{red}{\underline{0.04}} & 0.06 & 0.08 & 0.1 & 0.12 \\
% CIFAR-10 & precision & 0.74 & \textcolor{red}{\underline{0.89}} & 1.00 & 1.00 & 1.00 & 1.00 \\
% small & recall & 1.00 & \textcolor{red}{\underline{1.00}} & 0.75 & 0.75 & 0.72 & 0.62 \\
%  & \#TP & 32 & \textcolor{red}{\underline{32}} & 24 & 24 & 23 & 20 \\

% \midrule
% Robust& threshold & 0.015 & 0.03 & \textcolor{red}{\underline{0.045}} & 0.06 & 0.075 & 0.09 \\
% CIFAR-10 & precision & 0.73 & 0.82 & \textcolor{red}{\underline{0.97}} & 1.00 & 1.00 & 1.00 \\
% small & recall & 1.00 & 1.00 & \textcolor{red}{\underline{0.88}} & 0.75 & 0.75 & 0.72 \\
%  & \#TP & 32 & 32 & \textcolor{red}{\underline{28}} & 24 & 24 & 23 \\

% \midrule
% Robust& threshold & 0.015 & \textcolor{red}{\underline{0.03}} & 0.045 & 0.06 & 0.075 & 0.09 \\
% CIFAR-10 & precision & 0.73 & \textcolor{red}{\underline{0.78}} & 0.82 & 0.89 & 0.92 & 1.00 \\
% resnet & recall & 1.00 & \textcolor{red}{\underline{1.00}} & 0.88 & 0.78 & 0.72 & 0.59 \\
%  & \#TP & 32 & \textcolor{red}{\underline{32}} & 28 & 25 & 23 & 19 \\
% \bottomrule
% \end{tabular}

% {(\textbf{acd} threshold is 0.01 for \coco, \coco with gender, imSitu and \cifar; \textbf{acd} threshold is 0.001 for NUS and ImageNet; \textbf{acd} threshold is 0.05 for Robust cifar10 small, large, and resnet)}
% \end{table}




\begin{table}[!phtb]
%\begin{tabular}{l|l|cccccc}
\centering
\scriptsize
\caption{Accuracy in confusion errors detection (top 0.1 percentage)}
\label{tab:confusion_accuracy_1}
\begin{tabular}{l|l|rrrrr}
\toprule
dataset & model & tp & fp & precision & recall & f1 \\
\midrule
COCO & rand & 0.10 & 31 & 284 & 0.100 & 0.100 & 0.100 \\
COCO & ours & 148 & 168 & 0.468 & 0.468 & 0.468 \\
\midrule
COCO gender & rand  & 32 & 291 & 0.100 & 0.100 & 0.100 \\
COCO gender & ours  & 137 & 187 & 0.423 & 0.423 & 0.423 \\
\midrule

NUS & rand   & 4995 & 44955 & 0.100 & 0.100 & 0.100 \\
NUS & ours  & 21697 & 28253 & 0.434 & 0.434 & 0.434 \\
\midrule
CIFAR-100 & ran   & 46 & 449 & 0.093 & 0.093 & 0.093 \\
CIFAR-100 & ours  & 238 & 257 & 0.481 & 0.481 & 0.481 \\
\midrule
R CIFAR-10 S & rand  & 0 & 4 & 0 & 0 & 0 \\
R CIFAR-10 S & ours  & 3 & 1 & 0.75 & 0.75 & 0.75 \\
\midrule
R CIFAR-10 L& rand  & 1 & 3 & 0.25 & 0.25 & 0.25 \\
R CIFAR-10 L& ours  & 3 & 1 & 0.75 & 0.75 & 0.75 \\
\midrule
R CIFAR-10 R & rand  & 1 & 3 & 0.25 & 0.25 & 0.25 \\
R CIFAR-10 R & ours  & 3 & 1 & 0.75 & 0.75 & 0.75 \\
\midrule
R T ImageNet& rand   & 174 & 1816 & 0.087 & 0.087 & 0.087 \\
R T ImageNet& ours  & 731 & 1259 & 0.367 & 0.367 & 0.367 \\

\midrule
Imsitu& rand   & 53 & 452 & 0.105 & 0.105 & 0.105 \\
Imsitu& ours  & 227 & 278 & 0.45 & 0.45 & 0.45 \\
\bottomrule
\end{tabular}
%\vspace{-0.4cm}
\end{table}



==> tables/deepgaugecoverage.tex <==
\ \\
DeepGauge proposed five coverage criteria:

k-multisection neuron coverage, neuron boundary coverage and strong neuron activation coverage are neuron level coverage criteria. They requires obtaining each neuron's output boundary from training data to approximate the major function region and corner-case region.

From training data analysis, we can get the boundary $[{low}_n,{high}_n]$ for each neuron n as major function region and $(-\infty, {low}_n) \cup ({high}_n, +\infty)$ as corner-case region.

1) \textbf{k-multisection neuron coverage}\\
we first partition $[{low}_n,{high}_n]$ into k sections.\\
k-multisection neuron coverage of each neuron is defined as
$$
\frac{number~of~covered~ sections}{k}
$$

k-multisection neuron coverage of a DNN is defined as
$$
\frac{\sum_{i \in N}(number~of~covered~ sections~of~neuron~i)}{k \times |N|}
$$

2) \textbf{neuron boundary coverage}:\\
We first define a neuron's UpperCornerRegion as $({high}_n, +\infty)$ and its LowerCornerRegion as $(-\infty, {low}_n)$

neuron boundary coverage of a DNN is defined as
$$
\frac{|\{n|upper(n)~covered\}| + |\{n|lower(n)~covered\}|}{2 \times |N|}
$$

3) \textbf{strong neuron activation coverage}: \\

$$
\frac{|\{n|upper(n)~covered\}|}{|N|}
$$

Layer level coverage criteria:

1)\textbf{top-k neuron coverage}:
top-k neuron coverage is defined as the ratio of the total number of top-k neurons on each layer and the total number of neurons in a DNN given a set of test inputs


2)\textbf{top-k neuron patterns}.
top-k neuron patterns is defined as the number of top-k neuron patterns given a set of test inputs \\
$|\{top_k(x,1),...,top_k(x,l)|x\in T\}|$

a neuron pattern is a sequence from the topk neuron set of the first layer to the topk neuron set of the last layer.





==> tables/notation.tex <==
\begin{table}[h]
 % \vspace{-0.2cm}
    \scriptsize
    \small
    
    \caption{\textbf{\small Definitions we used to test a model}}
    \label{tab:notation}
    \centering
    \begin{tabular}{ll}
    \toprule
    All neurons set     & $ N = \{n_1,n_2,...\}$ \\ %\midrule
%    Training data set   & $ EC_{Train} = \{EC_1,EC_2,...\}$\\ %\midrule
    % Equivalence class   & $ EC_i = \{e_{i1},e_{i2}, ...\}$ \\
    %                     & where $ e_{ik}$ is an input from $EC_i$ \\     %\midrule
%    Test data set       & $ T = EC_{Test} = \{t_1,t_2,...\}$.  \\ %\midrule
    Activation function & $ out(n, c)$ returns output  \\ %\midrule
         & for neuron $ n$ , input $c$. \\ %\midrule
    Activation threshold & $Th$ \\
    \bottomrule
    \end{tabular}
    \vspace{-3mm}
\end{table}
